Quantifying Privacy Leakage in Graph Embedding

Graph embeddings have been proposed to map graph data to low dimensional space for downstream processing (e.g., node classification or link prediction). With the increasing collection of personal data, graph embeddings can be trained on private and sensitive data. For the first time, we quantify the privacy leakage in graph embeddings through three inference attacks targeting Graph Neural Networks. We propose a membership inference attack to infer whether a graph node corresponding to individual user's data was member of the model's training or not. We consider a blackbox setting where the adversary exploits the output prediction scores, and a whitebox setting where the adversary has also access to the released node embeddings. This attack provides an accuracy up to 28% (blackbox) 36% (whitebox) beyond random guess by exploiting the distinguishable footprint between train and test data records left by the graph embedding. We propose a Graph Reconstruction attack where the adversary aims to reconstruct the target graph given the corresponding graph embeddings. Here, the adversary can reconstruct the graph with more than 80% of accuracy and link inference between two nodes around 30% more confidence than a random guess. We then propose an attribute inference attack where the adversary aims to infer a sensitive attribute. We show that graph embeddings are strongly correlated to node attributes letting the adversary inferring sensitive information (e.g., gender or location).

==> mitigation.tex <==
\section{Mitigating Privacy Risks}\label{discuss}

We discuss some potential mitigation strategies to lower the privacy risks from the proposed algorithms and keep the evaluations as future work.

\noindent\textbf{Lower Embedding Precision.} The embeddings are continuous values and capture the semantic information about the graph structure.
These embeddings while reduce the overall dimensionality of the graph data also capture rich information about the input graphs by ensuring that the properties in the graph are still maintained in the embedding.
Lowering the precision of the embedding vector for each node by rounding can help reduce the attack model from learning rich features about the inputs~\cite{membershipinf,nlp}.

\noindent\textbf{Adversarial Examples.} In the proposed attacks, the attacker model typically involves a machine learning algorithm (e.g node and attribute inference, decoder for graph reconstruction).
Adversarial examples are imperceptible noise added to the output prediction to force the target model to misclassify.
Since, the attack models are vulnerable to adversarial examples, the released embedding can be released with an additional adversarial noise to misclassify the target model.
However, the noise added to be optimized to ensure utility for further downstream applications~\cite{attriguard,memguard}.

\noindent\textbf{Adversarial Training.} In case of node membership inference can be modelled as an minimax adversarial training with joint optimization to minimize the model loss using the graph embeddings (e.g GNNs) while maximising the adversary's loss on inferring the sensitive inputs.
Such a joint optimization can be used to update the embeddings such that they maintain the original graph properties while ensuring that the attack model performance is low.
For inference time, such defences have been explored in the context of traditional machine learning to protect against membership inference~\cite{advreg} and preserve privacy of text models~\cite{textembleak}.

\noindent\textbf{Differential Privacy.} One major approach to protect an individual user's privacy is to add noise sampled from Laplacian and Gaussian distribution.
This carefully added noise ensures that the presence or absence of a user's data in the mechanism does not change the model output.
Further, DP provides a theoretical bound on the total privacy leakage from the mechanism (downstream processing from embeddings) on an individual's data point.
Such DP based embeddings have been proposed for both graph and text models~\cite{dptext,dpne}, however, their efficacy against the proposed privacy attacks are yet to be studied as part of the future work.

